All-sky spectroscopic survey of bright {\delta} Scuti stars from TESS Projected rotational velocities and pulsation characteristics

Context. The second most numerous class of pulsating stars -- $\delta$ Scuti ($\delta$ Sct) -- lack a homogeneous, large-scale spectroscopic sample in the Kepler and TESS era, limiting our understanding of how rotation shapes stellar pulsations. Aims. We analyse projected rotational velocities ($v \sin i$) from high-resolution spectroscopy alongside 2-minute TESS photometry to establish empirical links between stellar rotation and pulsation parameters. Methods. Combining observations from three high-resolution \'echelle spectrographs with two spectral libraries, we assemble an all-sky sample of 262 $\delta$ Sct stars ($R = 25\,000$ to $115\,000$). We derive $v \sin i$ via three independent methods and extract pulsation frequencies and amplitudes from TESS light curves. Results. The $v \sin i$ distribution is unimodal, with a mean of $120.3\text{ km s}^{-1}$ and peak probability at $113.8\text{ km s}^{-1}$. Minimum ($\nu_{\rm min}$), dominant ($\nu_{\rm dom}$), amplitude-weighted ($\nu_{\rm AW}$), and power-weighted ($\nu_{\rm PW}$) frequencies decrease with $v \sin i / v_{\rm crit}$, whereas maximum frequency ($\nu_{\rm max}$) does not. Fast rotators show a narrower range of photometric and pulsation amplitudes than slow rotators, and their lower mean stellar density ($\bar{\rho}$) cannot fully explain the frequency decrease. Calibrating Gaia's $v_{\rm broad}$ against our measurements removes its systematic offset, enabling use across larger $\delta$ Sct samples. Multi-spectrum comparisons reveal method discrepancies mainly for fast rotators ($v \sin i > 200\text{ km s}^{-1}$) and inter-spectrograph offsets up to $20\text{ km s}^{-1}$. Conclusions. We present the largest homogeneous high-resolution $v \sin i$ sample for bright $\delta$ Sct stars in the TESS era, showing that $v \sin i$ measurements in pulsating stars require careful treatment across instruments and velocity regimes.

==> bibtex/bibliography.tex <==
%%% Bibliography (literature used as a source)
%%%
%%% We employ biblatex to construct the bibliography. It processes
%%% citations in the text (e.g., the \cite{...} macro) and looks up
%%% relevant entries in the bibliography.bib file.
%%%
%%% See also biblatex settings in thesis.tex.

%%% Generate the %%% Bibliography (literature used as a source)
%%%

%%% use \citep Harmanec (2022) and \citet (Harmenac, 2022), not \cite

%%% I have copied citation style from Astronomy and Astrophysics
\bibliographystyle{aa}
\bibliography{bibliography.bib}

